CRScore++: Reinforcement Learning with Verifiable Tool and AI Feedback for Code Review

Reinforcement learning (RL) to improve code review comment generation requires handling unstructured outputs, making reinforcement learning (RL) feedback challenging. The two main RL approaches, namely RL with Verifiable Feedback (RLVR) and RL with AI Feedback (RLAIF), offer trade-offs: RLVR provides reliable feedback for structured tasks like code generation, while RLAIF works for unstructured outputs but is subjective. We bridge this gap with CRScore++, an RL framework that leverages both LLM-based subjective feedback and verifiable signals for training. Extending CRScore, a code review evaluation metric integrating LLMs with verifiers like linters and code smell detectors, CRScore++ transforms these signals into training rewards. We show that CRScore++ improves a weaker student model through a combination of supervised fine-tuning and RL critique from a stronger teacher model, thus enabling generalization to novel programming languages.

==> Chapters/Abstracts/abstract_v1.tex <==
Recent advances in reinforcement learning (RL) training for tasks like code generation have successfully leveraged verifiable rewards like execution feedback at scale.
Despite their promise, verifiable rewards are hard to apply for natural language generation (NLG) domains like code review comment generation.
Subsequently, RL for NLG tasks has traditionally relied on learning from human feedback (RLHF) or AI feedback (RLAIF), which relies on subjective preference signals. 
However, this does not mean that feedback from domain-specific verifiers can't be incorporated as training signals.
In this paper, we propose an RLAIF paradigm called CRScore++ that extends CRScore, an existing evaluator based on LLMs combined with code review-specific verifiers like code smell detectors, linters, and security analyzers.
We show that CRScore++ can be used to improve a weaker student model for the task of code review with both demonstrations (supervised fine-tuning) and critique (RL) from a stronger teacher model.
Additionally, CRScore++ can teach the student model to generalize knowledge learned from the verifiers during training to novel programming languages during test time.

==> Chapters/Abstracts/abstract_v2.tex <==
The two most common reinforcement learning (RL) approaches for code models are RL with Verifiable Feedback (RLVR) and RL with AI Feedback (RLAIF). RLVR provides reliable and objective feedback for structured outputs like code, whereas RLAIF works for unstructured outputs but is subjective and less reliable.
In this paper, we combine the strengths of both methods by introducing CRScore++ for code review comment generation--- a task with unstructured outputs--- by leveraging both the subjective feedback of Large Language Models (LLMs) and verifiable signals. Our approach extends CRScore, a code review evaluation metric that integrates LLMs with code review-specific verifiers such as code smell detectors and linters, transforming it into a training signal.
We demonstrate that CRScore++ can enhance a weaker student model for code review through both demonstrations (supervised fine-tuning) and critique (RL) from a stronger teacher model. Moreover, we show that CRScore++ enables the student model to generalize knowledge from verifiers during training to novel programming languages at test time.

==> Chapters/Chapter1_Introduction.tex <==
\section{Introduction}
\label{Chapter 1}

In recent years, large language models (LLMs) have been increasingly adopted for software engineering tasks \cite{zhang2023unifying}. 
This has been partly fueled by advancements in reinforcement learning (RL)-based training methods, especially ones that incorporate verifiable rewards (RLVR) like execution feedback \cite{codeRL, dou2024stepcoderimprovecodegeneration, shojaee2023executionbasedcodegenerationusing}.
While these learning signals have been successfully applied for tasks with structured outputs like code, developing and applying verifiable rewards is challenging for natural language generation (NLG) tasks like code review.
For NLG tasks, the research community has primarily relied on supervised fine-tuning (SFT) with high-quality examples, RL from human feedback (RLHF) \cite{rlhf}, or from AI feedback (RLAIF) \cite{rlaif} for greater scalability. 
While RLVR is scalable and verifiable, RLHF and RLAIF, rely on subjective preference signals \cite{openai2024gpt4, bai2022constitutionalaiharmlessnessai} which can lead to unintentional biases in models.
However some of these biases may be desirable as shown by studies on using LLM-as-a-judge (a form or RLAIF), for software engineering \cite{he2025codecourtroomllmsnew, wang2025llmsreplacehumanevaluators} indicating high agreement and similar score distributions to human evaluators.
Moreover, for an NLG domain like code review, RLVR is hard to apply due to the free form text output.
Consequently recent works have demonstrated the benefits of combining LLMs with verifiable static analysis tools, such as linters and code smell detectors, at test time or for data generation for both evaluating review comments \cite{crscore_paper} and generating them \cite{jaoua2025combininglargelanguagemodels}.
Drawing inspiration from these works, we take steps towards leveraging verifiers for training by incorporating verifiable ``facts'' from static analysis tools along with more subjective LLM feedback (RLAIF), leading to a new training framework called CRScore++.

Our training framework involves two stages: (1) learning from demonstrations (SFT) and (2) learning from critique (Preference Optimization or PO), with both stages incorporating ``facts'' generated by verifiers in step-by-step reasoning.
The SFT stage leverages a stronger teacher model to generate demonstrations or code review comments for a student model via a chain of thought (CoT) that integrates relevant linter messages and code smells into the target review label.
This follows from recent work that shows incorporating tools can help improve the reasoning abilities of reasoning models \cite{li2025startselftaughtreasonertools}.
Meanwhile, the PO stage uses the teacher model as a ``critique'' for the review comments generated by the student model by first generating a list of things the review should address (pseudo-references generated by CRScore \cite{crscore_paper}) that includes the tool outputs and then generating a CoT to determine which of these are addressed in the student model's review. 
Based on the findings of \cite{sharma2024criticalevaluationaialign}, we use the same teacher model for the SFT and PO stages.
Apart from the benefit of grounding RLAIF with verifiable facts from tools, we also indirectly train the model to detect code smells and linter related issues through the CoT.
This can lead to generalization of these abilities across programming languages, where we can train the model with tool feedback for just one language like Python and generalize these abilities to other languages like Java and Javascript during inference.
We speculate that this could be facilitated by systematically applying or unlocking the model's knowledge about these languages acquired during pre-training.

Our work makes three primary contributions:
\begin{itemize}[noitemsep,topsep=0pt,leftmargin=*]
    \item Introducing a novel RL method for code model training that combines benefits of RLVR with the flexibility of RLAIF.
    \item Applying this framework to integrate linters, code smell detectors, security analyzers, etc., into code review model training--a first, to the best of our knowledge.
    \item Facilitating learning of skills like code smell detection, evaluating code efficiency, security, readability, maintainability etc. in a generalizable way across programming languages via step by step reasoning.
\end{itemize}

% Current state-of-the-art approaches for enhancing code generation capabilities have explored various reinforcement learning techniques. StepCoder \cite{dou2024stepcoderimprovecodegeneration} addresses exploration challenges by breaking long sequence code generation into a curriculum of code completion subtasks while providing fine-grained optimization by masking unexecuted code segments. CodeRL \cite{le2022coderl} leverages execution feedback in a reinforcement learning framework, treating the code-generating LLM as an actor network and introducing a critic network trained to predict functional correctness. PPOCoder \cite{shojaee2023executionbasedcodegenerationusing} combines pre-trained programming language models with Proximal Policy Optimization to integrate external code-specific knowledge into model optimization. While these approaches have shown promising results, they primarily focus on code generation rather than code review, and most rely on execution-based feedback rather than static analysis, which limits their applicability to code that cannot be easily executed or where runtime behavior is not the primary concern.

% More recent work has begun exploring the integration of static analysis tools with LLMs. 
% CodePatchLLM \cite{shaikhelislamov2024codepatchllm} proposes a novel approach that utilizes a static analyzer tool to enhance the reliability and security of generated code, demonstrating improvements in compilation rates and functional correctness across different programming languages. 
% However, this approach focuses on iteratively correcting model prompts rather than incorporating static analysis feedback directly into the reinforcement learning process. 
% Focused-DPO \cite{zhang2025focuseddpoenhancingcodegeneration} identifies that current models tend to produce errors concentrated at specific error-prone points and introduces a framework that enhances code generation by directing preference optimization toward these critical areas. 
% While this approach improves precision and reliability, it does not fully leverage deterministic feedback from static analysis tools. 

% Our work bridges the gap between SFT and SFT+DPO approaches by incorporating verifiable rewards from linters such as ruff and static analyzers into the reinforcement learning process for code review tasks. 
% Unlike prior work that primarily focuses on code generation, we target the task of generating high-quality code reviews that incorporate feedback from static analysis tools. 
% This builds upon the emerging paradigm of Reinforcement Learning with Verifiable Rewards (RLVR) \cite{RLVR}, which enables objective optimization through programmatic validation. While verifiable rewards have been extensively explored for mathematical reasoning and code execution, their application to code review tasks utilizing static analysis tools remains underexplored \cite{lambert2025tulu3pushingfrontiers}. 
% Our approach combines linter outputs, code smell detectors, and security analysis tools into a composite reward signal, overcoming the manual verification bottleneck observed in prior systems. We leverage Group Relative Policy Optimization (GRPO) techniques, similar to those employed by DeepSeek R1 \cite{deepseekai2025deepseekr1incentivizingreasoningcapability}, while introducing tool-guided reward shaping for improved sample efficiency.

%TODO: one point should be about verifiable rewards in NLG/RLAIF, one point should be about cross-language generalization of tool knowledge without explicit training, and one point should be about incoporating tools as reward signals into code review comment generation training (probably first point), while other works have only explored data augmentation.
% (1) We introduce a novel framework that integrates verifiable rewards from static analysis tools like linters and code smell detectors
% such as ruff \footnote{\url{https://github.com/astral-sh/ruff}} and Pyscent \footnote{\url{https://github.com/whyjay17/Pyscent}} 
% directly into the SFT and PO stage via chains of thought for code review comment generation, an approach not previously explored in the training of LLMs of Code. Second, we demonstrate generalization across programming languages via test-time adaptation to Java and JavaScript through smells and linters messages despite the lack of explicit training with static analysis tools for them. This cross-language transfer suggests that our approach captures fundamental code quality principles that transcend specific language syntax. Third, we produce an enhanced model for code review that incorporates signals from static analysis tools, bridging a gap in current research that has extensively explored this approach for code generation but has given less attention to natural language feedback generation in code review contexts. Our comprehensive evaluation methodology includes both automated metrics and human evaluation, providing a thorough assessment of our approach's effectiveness compared to traditional SFT-only methods.


==> Chapters/Chapter3_Dataset_Collection.tex <==
% Chapter Template
\section{Dataset Description} % Main chapter title

\label{Chapter3} % Change X to a consecutive number; for 



==> Chapters/supplementary_material.tex <==
\section{Appendix}
\label{Chapter_supplementary}

% \begin{figure*}[!tbhp]
% \centering
% \includegraphics[width=2\columnwidth]{images/CRScore++ Evaluation new.png}
% \caption{Evaluation framework combining static verification with LLM-as-judge}
% \label{fig:evaluation_llm_as_a_judge}
% \end{figure*}

\begin{table*}[htbp]
\centering

\resizebox{2\columnwidth}{!}{\begin{tabular}{l 
                cc   cc   cc}
\toprule
Comparison 
  & \multicolumn{2}{c}{Comprehensiveness} 
  & \multicolumn{2}{c}{Conciseness} 
  & \multicolumn{2}{c}{Relevance} \\

  & p-value & statistic 
  & p-value & statistic 
  & p-value & statistic \\

\midrule
Qwen 3B (CR dataset\textsubscript{\texttt{Python only}}) vs. Qwen 7B (CR dataset\textsubscript{\texttt{Python only}}) 
  & \textbf{p<0.01} & 7.50e+06 
  & p>0.01 & 8.07e+06 
  & \textbf{p<0.01} & 7.50e+06 \\

Qwen 3B Zero Shot vs.\ Qwen 7B Zero Shot
  & p>0.01 & 8.34e+06 
  & \textbf{p<0.01 }& 8.67e+06 
  & \textbf{p<0.01} & 8.49e+06 \\

Qwen 3B (Tool Guided)  
   vs.\ Qwen 7B (Tool Guided)
  & p>0.01 & 8.17e+06 
  & \textbf{p<0.01} & 8.57e+06 
  & p>0.01 & 8.25e+06 \\

Qwen 3B Stage 1 vs.\ Qwen 7B Stage 1
  & \textbf{p<0.01} & 8.71e+06 
  & \textbf{p<0.01} & 7.73e+06 
  & \textbf{p<0.01} & 8.64e+06 \\

Qwen 3B Stage 2 vs.\ Qwen 7B Stage 2
  & \textbf{p<0.01} & 7.32e+06 
  & \textbf{p<0.01} & 8.75e+06 
  & \textbf{p<0.01} & 7.28e+06 \\

\bottomrule
\end{tabular}}
\caption{Statistical significance Wilcoxon Signed Rank tests performed among Qwen 3B and 7B variants on comprehensiveness, conciseness, and relevance (significance level $\alpha = 0.01$). We highlight statistically significant observations.}
\label{tab:size-comparison}
\end{table*}

\begin{table*}[htbp]
\centering
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{l  cc  cc  cc}
\toprule
Comparison 
  & \multicolumn{2}{c}{Comprehensiveness} 
  & \multicolumn{2}{c}{Conciseness} 
  & \multicolumn{2}{c}{Relevance} \\

  & p-value & statistic 
  & p-value & statistic 
  & p-value & statistic \\

\midrule
Qwen 3B (CR dataset\textsubscript{\texttt{Python only}}) vs.\ Qwen 3B Zero Shot  
  & \textbf{p<0.005} & 1.48e+06 
  & \textbf{p<0.005} & 5.65e+06 
  & \textbf{p<0.005} & 2.57e+06 \\

Qwen 3B (CR dataset\textsubscript{\texttt{Python only}}) vs.\ Qwen 3B (Tool Guided)  
  & \textbf{p<0.005} & 1.70e+06 
  & \textbf{p<0.005} & 5.62e+06 
  & \textbf{p<0.005} & 2.82e+06 \\

Qwen 3B (CR dataset\textsubscript{\texttt{Python only}}) vs.\ Qwen 3B Stage 1  
  & \textbf{p<0.005} & 4.07e+05 
  & \textbf{p<0.005} & 5.69e+06 
  & \textbf{p<0.005} & 1.20e+06 \\

Qwen 3B (CR dataset\textsubscript{\texttt{Python only}}) vs.\ Qwen 3B Stage 2  
  & \textbf{p<0.005} & 2.56e+05 
  & \textbf{p<0.005} & 7.38e+06 
  & \textbf{p<0.005} & 8.48e+05 \\

Qwen 3B Zero Shot vs.\ Qwen 3B (Tool Guided) 
  & \textbf{p<0.005} & 8.40e+06 
  & p>0.005 & 8.07e+06 
  & \textbf{p<0.005} & 8.42e+06 \\

Qwen 3B Zero Shot vs.\ Qwen 3B Stage 1  
  & \textbf{p<0.005} & 4.77e+06 
  & p>0.005 & 8.17e+06 
  & \textbf{p<0.005} & 5.36e+06 \\

Qwen 3B Zero Shot vs.\ Qwen 3B Stage 2  
  & \textbf{p<0.005} & 3.39e+06 
  & \textbf{p<0.005} & 1.00e+07 
  & \textbf{p<0.005} & 4.02e+06 \\

Qwen 3B (Tool Guided) vs.\ Qwen 3B Stage 1  
  & \textbf{p<0.005} & 4.60e+06 
  & p>0.005 & 8.21e+06 
  & \textbf{p<0.005} & 5.11e+06 \\

Qwen 3B (Tool Guided) vs.\ Qwen 3B Stage 2  
  & \textbf{p<0.005} & 3.28e+06 
  & \textbf{p<0.005} & 1.01e+07 
  & \textbf{p<0.005} & 3.82e+06 \\

Qwen 3B Stage 1 vs.\ Qwen 3B Stage 2  
  & \textbf{p<0.005} & 6.30e+06 
  & \textbf{p<0.005} & 9.98e+06 
  & \textbf{p<0.005} & 6.51e+06 \\

\bottomrule
\end{tabular}%
}
\caption{Statistical significance Wilcoxon Signed Rank tests performed among Qwen 3B variants on comprehensiveness, conciseness, and relevance (significance level $\alpha = 0.005$). We highlight statistically significant observations.}
\label{tab:qwen3b-variants-significance}
\end{table*}


\begin{table*}[h]
\centering
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{l  cc  cc  cc}
\toprule
Comparison 
  & \multicolumn{2}{c}{Comprehensiveness} 
  & \multicolumn{2}{c}{Conciseness} 
  & \multicolumn{2}{c}{Relevance} \\

  & p-value & statistic 
  & p-value & statistic 
  & p-value & statistic \\

\midrule
Qwen 7B (CR dataset\textsubscript{\texttt{Python only}}) vs.\ Qwen 7B Zero Shot  
  & \textbf{p<0.005} & 2.82e+06 
  & \textbf{p<0.005} & 6.45e+06 
  & \textbf{p<0.005} & 4.03e+06 \\

Qwen 7B (CR dataset\textsubscript{\texttt{Python only}}) vs.\ Qwen 7B (Tool Guided)
  & \textbf{p<0.005} & 2.87e+06 
  & \textbf{p<0.005} & 6.31e+06 
  & \textbf{p<0.005} & 4.05e+06 \\

Qwen 7B (CR dataset\textsubscript{\texttt{Python only}}) vs.\ Qwen 7B Stage 1  
  & \textbf{p<0.005} & 7.67e+05 
  & \textbf{p<0.005} & 5.31e+06 
  & \textbf{p<0.005} & 1.74e+06 \\

Qwen 7B (CR dataset\textsubscript{\texttt{Python only}}) vs.\ Qwen 7B Stage 2  
  & \textbf{p<0.005} & 7.20e+05 
  & p>0.005 & 8.01e+06 
  & \textbf{p<0.005} & 1.31e+06 \\

Qwen 7B Zero Shot vs.\ Qwen 7B (Tool Guided)  
  & p>0.005 & 8.15e+06 
  & p>0.005 & 7.99e+06 
  & p>0.005 & 8.13e+06 \\

Qwen 7B Zero Shot vs.\ Qwen 7B Stage 1  
  & \textbf{p<0.005} & 5.37e+06 
  & \textbf{p<0.005} & 7.27e+06 
  & \textbf{p<0.005} & 5.74e+06 \\

Qwen 7B Zero Shot vs.\ Qwen 7B Stage 2  
  & \textbf{p<0.005} & 3.19e+06 
  & \textbf{p<0.005} & 9.80e+06 
  & \textbf{p<0.005} & 3.63e+06 \\

Qwen 7B (Tool Guided) vs.\ Qwen 7B Stage 1  
  & \textbf{p<0.005} & 5.36e+06 
  & \textbf{p<0.005} & 7.41e+06 
  & \textbf{p<0.005} & 5.73e+06 \\

Qwen 7B (Tool Guided) vs.\ Qwen 7B Stage 2  
  & \textbf{p<0.005} & 3.23e+06 
  & \textbf{p<0.005} & 9.96e+06 
  & \textbf{p<0.005} & 3.64e+06 \\

Qwen 7B Stage 1 vs.\ Qwen 7B Stage 2  
  & \textbf{p<0.005} & 5.10e+06 
  & \textbf{p<0.005} & 1.09e+07 
  & \textbf{p<0.005} & 5.32e+06 \\

\bottomrule
\end{tabular}%
}
\caption{Statistical significance Wilcoxon Signed Rank tests performed among Qwen 7B variants on comprehensiveness, conciseness, and relevance (significance level $\alpha = 0.005$). We highlight statistically significant observations.}
\label{tab:qwen7b-variants-significance}
\end{table*}



% 3. Run⁠ ⁠⁠language wise accuracy and coverage for 70 samples each language and run it using GPT4o ->  python only language take 100 instance 70*6 settings - > 420 
% java and js in that case take zero shot 70
% similarly java and js -> take 0 each language each setting and evaluate.

% Python (70): 3/7B S1/S2/Tools
% Java (70): 3/7B S1/S2/Zero Shot
% Javascript (70): 3/7B S1/S2/Zero Shot

% 4. add this to discussion: we are assuming that you will not always have access to tools for all languages, we will simulate the settings such that a user has access to python tools and not java and js tools, that's why fr both training setting and zero shot with tools, we dont give python in output, whereas giving for java and js.


% Table1 -> Find out reason why 3B and 7B zero shot performance, why is 3B always worse, check.

% [4/22/25, 11:44:00 PM] Atharva Naik Roshan IIT KGP: 3B > 7B for all untrained settings
% for some trained settings like CodeReviewer data and Stage 2: 7B has more Comp and Rel
% for stage 1: 3B has more Comp and Rel
% when Comp is greater conciseness is lower and when Comp is higher Rel is higher
% Stage 2 leads to more Comp and lower Con - can we explain this using "Final Review" length
% [4/22/25, 11:44:55 PM] Atharva Naik Roshan IIT KGP: Stage 2 leads to more Comp and lower Con - can we explain this using "Final Review" length - check if this is because the Final Review is on average longer in Stage 2 trained models compared to Stage 1 models.
